Analysing Lightweight Large Language Models for Biomedical Named Entity Recognition on Diverse Ouput Formats

Despite their strong linguistic capabilities, Large Language Models (LLMs) are computationally demanding and require substantial resources for fine-tuning, which is unadapted to privacy and budget constraints of many healthcare settings. To address this, we present an experimental analysis focused on Biomedical Named Entity Recognition using lightweight LLMs, we evaluate the impact of different output formats on model performance. The results reveal that lightweight LLMs can achieve competitive performance compared to the larger models, highlighting their potential as lightweight yet effective alternatives for biomedical information extraction. Our analysis shows that instruction tuning over many distinct formats does not improve performance, but identifies several format consistently associated with better performance.

==> latex/related-work-long.tex <==
Information extraction (IE) has witnessed significant advances with the advent of large language models (LLMs) and unified generation frameworks. Universal Information Extraction (UIE)~\cite{0001LDXLHSW22} proposes a unified text-to-structure generation framework, introducing a Structural Extraction Language to represent diverse IE structures and a Structural Schema Instructor to guide adaptive structure generation. Pre-trained on large-scale heterogeneous web data, UIE demonstrates effective knowledge transfer across supervised, low-resource, and few-shot settings. Similarly, \cite{corr/abs-2304-08085} reformulates IE as a natural language generation problem guided by descriptive task instructions. The method constrains the output space via an option mechanism covering all candidate categories and leverages auxiliary tasks such as span typing for NER, pair extraction for RE, and trigger-argument extraction for EE, enhancing structural and semantic understanding.

Zero-shot information extraction (ZIE)~\cite{corr/abs-2302-10205} aims to build systems without annotated data, significantly reducing labeling effort. Inspired by LLM advances such as GPT-3 and ChatGPT, ChatIE reformulates ZIE as a multi-turn question-answering problem using a two-stage framework. Evaluated across entity-relation extraction, NER, and EE tasks in multiple languages, ChatIE achieves strong performance, even surpassing some fully supervised models, highlighting the potential of resource-efficient IE.

LLMs with code-style prompts have shown notable success in IE. Code4UIE~\cite{GuoLJLZLLYBGC24} addresses challenges of non-unified prompts and limited in-context learning by introducing a Python class–based schema that standardizes diverse IE tasks and integrates retrieval-augmented mechanisms. Similarly, \cite{talip/BiCJXGCZ24} frame generative knowledge graph construction as a code completion task with schema-aware prompts and rationale-enhanced generation, improving extraction accuracy. GoLLIE~\cite{iclr/SainzGALRA24} fine-tunes LLMs to attend to annotation guidelines across small sets of IE tasks, demonstrating the benefit of task-specific instruction tuning.

\paragraph{Data Annotation} LLMs have been employed to generate labeled data efficiently. LLMaAA~\cite{ZhangLMZ023} improves annotation and training efficiency by using LLMs as annotators within an active learning loop, reducing dependence on manual labeling. \cite{WangZQLL23} enhances unsupervised RE by augmenting sentence pairs and incorporating a margin loss to improve model discrimination between positive and negative examples.

\paragraph{Knowledge Retrieval} Retrieval-augmented methods leverage LLMs as implicit knowledge bases. Li et al.~\cite{LiLPSWZP23} introduce a two-stage multimodal NER framework that heuristically retrieves auxiliary refined knowledge to improve entity prediction. \cite{AmalvyLD23} generate synthetic context datasets and train neural retrievers to support NER on long documents. Chain-of-Thought Prompt Distillation~\cite{corr/abs-2306-14122} integrates text–image pairs with CoT reasoning and applies data augmentation to enhance cross-modal NER and RE performance.

\paragraph{Inverse Generation} Reversing the task direction to generate text from structured data has been explored in multiple works. SynthIE~\cite{JosifoskiSP023} generates high-quality synthetic data by inverting task inputs, enabling downstream models to outperform prior benchmarks. STAR~\cite{corr/abs-2305-15090} generates event extraction passages from structured triggers and arguments using LLMs with iterative refinement, preserving textual coherence and entity integrity. \cite{HuJLHXHWY23} employ entity-to-text augmentation by manipulating entity lists and applying diversity beam search to enhance dataset richness for NER.

\paragraph{Synthetic Datasets for Fine-tuning} Instruction-tuning benefits from LLM-generated synthetic datasets. UniversalNER~\cite{Zhou00CP24} distills ChatGPT into smaller student models using mission-focused instruction tuning for open NER. Rethinking Negative Instances~\cite{DingLWTBZ24} introduces negative examples to generative NER, training on Pile-NER with 240K entities across 13K categories, improving zero-shot performance on unseen entity domains.

\paragraph{Question Answering} QA-based prompting has been applied to enhance LLM reasoning in IE. Li et al.~\cite{LiWK23} propose a summarize-and-ask strategy to transform zero-shot RE into recursive QA, effectively handling none-of-the-above relations.

\paragraph{Chain-of-Thought} CoT prompting guides LLMs with step-wise reasoning. Zero-shot Temporal Relation Extraction with ChatGPT~\cite{YuanXA23} uses a two-stage approach to guide temporal relation reasoning, leveraging zero-shot capabilities without task-specific supervision.

\paragraph{Self-Improvement} LLMs can iteratively refine outputs through self-reflection. ProgGen~\cite{HengDLYLZZ24} guides LLMs to self-reflect, generate domain-relevant attributes, and proactively construct NER context data around entities, enhancing dataset quality.

\paragraph{Zero-shot Learning} Conditional generation approaches have been applied to unseen tasks. Li et al.~\cite{LiJH21} propose a document-level neural model for event argument extraction with strong portability to unseen event types, demonstrating robust cross-domain applicability.

\paragraph{Constrained Decoding Generation} Structured decoding improves output consistency. Geng et al.~\cite{GengJP023} introduce grammar-constrained decoding with input-dependent grammars to control LLM outputs for structured NLP tasks. Zaratiana et al.~\cite{ZaratianaTHC24} propose a text-to-graph framework generating linearized graphs for joint entity and relation extraction with a transformer encoder-decoder, a pointing mechanism, and dynamic vocabulary.

\paragraph{Few-shot Learning} Handling multiple domains with limited data has been explored in several works. Paolini et al.~\cite{PaoliniAKMAASXS21} unify structure generation for diverse IE tasks. Chen et al.~\cite{ChenLQ0TJHC23} use collaborative domain-prefix tuning for cross-domain NER. CodeIE~\cite{LiSTYWHQ23} converts IE tasks into code generation using code-style prompts and in-context examples, achieving superior few-shot performance.

\paragraph{Supervised Fine-tuning} LLM pretraining and distillation enhance structured task performance. DeepStruct~\cite{WangLCH0S22} pretrains LMs on task-agnostic corpora to improve structural understanding. UniversalNER~\cite{Zhou00CP24} distills ChatGPT into smaller student models for open NER, retaining performance while reducing model size. GIELLM~\cite{corr/abs-2311-06838} fine-tunes LLMs on mixed datasets for Japanese IE, leveraging mutual reinforcement effects to improve performance across multiple tasks.

Overall, these works highlight multiple complementary strategies for advancing IE, including data annotation with LLMs, knowledge retrieval, inverse generation, synthetic dataset construction, QA-based and chain-of-thought prompting, constrained decoding, few-shot adaptation, and supervised fine-tuning. Together, they demonstrate the growing potential of large language models to unify and enhance structured information extraction across languages, modalities, and domains.

==> latex/trash.tex <==
\ac{as tu fait expres de ne pas les mettre dans l'ordre d'apparition?}
\pe{Nan c'est GENIA qui ordonne comme ca. J'avoue que j'ai jamais fait attention. C'est une erreur, surtout parcequ'on finetune ...}


\ac{pourquoi dans ton prompt format n'est pas accompagné de langues naturel : ex: Please output the result in the \textit{format} format?}
\pe{
Parce que la phrase change un peu en fonction des formats. 

Pour code tu auras: You must answer by completing the code below.
Pour bio: "You must answer using the BIO format."
Pourterm 
Pour term: "You must answer by providing a list of string, with each string representing an entity."

Vu que j'utilise des modèles déjà instruct (pour la conversation) j'ai utilisé des phrases pour représenté les formats (et pour m'aligner sur ce qui est fait avec les formats venant d'autres sources aussi) De toute manière on finetune le modèle donc le prompt enginering a moins d'influence. Une des experiences qu'on avait envisager c'était de tester sans modèle instruct.

Dataset: {dataset}
Format: {Format}
Text: {text}
Entities: 

}
% \ac{on dirait que c'est multiple\_span non ? Car je vois trois spans qui correspondent à ta proteine et tes deux types cellulaires, non ? - sauf si single term veut dire term seulement et single span veut dire span seulement. Si c'est le cas il faut les appeler term\_only et span\_only}


%In this work, a \emph{format} defines how NER results are represented. This implies that each format specifies a distinct structure for representing entity terms and types. BIO (Beginning, Inside, Outside) is an example of format that is mainly used with model that solve NER using token classification. 

% \subsubsection{Entity Representations.}
% \ac{je crois que les choses sont males présentées ici. I ly a un probleme notamment car modalité et format me semble 2 choses différentes. Alors il faut peut etre distinguer les deux et modalities peut simplement etre 3.3. Est ce que tu as pensé a faire quelque chose de plus binaire, un peu comme dans le tableau 1 : 1) embedded vs extracted
% 2) extracted with span vs extracted without span
% - j'imagine que l'on a toujours l type}
% \paragraph{Text Reconstruction.}
% Entity terms and types are embedded within the text (e.g., using tags around entity mentions). Therefore, the model should generate a reconstructed version of the text with the appropriate modifications.

% \paragraph{Term Extraction.} 
% \ac{ceci s'appelle String Extraction dans le tableau...}
% Entity terms and types are extracted from the text and the term is represented as itself. Therefore, the model should generate a list of term and type.
% \ac{du coup dans ce cas, si on a uniquement la sortie, on ne sait pas ou sont les termes, il faut les chercher soit meme ? c'est ça ?}
% \paragraph{Span Extraction.}
% Entity terms and types are extracted from the text and the term is represented as a character span (start and end indices of the term). Therefore, the model should generate a list of spans and terms. \ac{ le dernier mot est peut etre "type", non ? sinon on  a gagné le span, mais perdu le type et du coup je ne comprends plus rien. D'autant que tu as dans Table 1 un format qui extrait span mais pas term/string}

% \ac{c'est quand meme très mal nommé ou expliqué ou les deux : est ce que span extraction n'est qu'une extension de term extraction? Est ce qu'on a pas le type dans span extraction? Si on reecrit les termes dans span extraction ?  Les termes Reconstruction et Extraction sont également assez mal choisi. }

% \subsubsection{Modalities.}

% \paragraph{Multi.}
% The format supports multiple entity types simultaneously. Each text is processed once, with the model receiving the complete list of entity types to extract in a single pass.
% \ac{ici tu mélanges le format en lui meme et le systeme qui reconnait un type ou plusieur types d'entité. Et c'est du coup dur a comprendre.}

% \paragraph{Single.}
% The format handles one entity type at a time. Consequently, each text is processed separately for every entity type to be extracted. % \textit{(If conflict evaluation is included, it can be mentioned here.)} \ma{what do you mean by conflicted evaluation.}

% \paragraph{Conversational.}
% This format supports multiple entity types by extracting each type in a separate turn, following a conversational interaction pattern.

% \ac{la on ne comprends pas bien pourquoi on ne pourrait pas avoir un single type conversational}

% \subsubsection{Format Selection}

% We choose our formats to maximize coverage of existing variants. %An example of each format can be find in appendix \ref{}. 
% Each of the format selection choice is described below and example given are related to the following user prompt: \ma{pierre is it repeating paragraph?}
% entity original terms \ma{surface forms?}, its type and potential\ma{?}  span. %For instance, the BIO (Beginning, Inside, Outside) format is commonly used to represent entities in  annotated corpora used for training and testing supervised NER. We choose these formats to maximize coverage of existing variants. Each of the format selection choice is described below and example given are related to the following user prompt:



%An example of each format can be find in appendix \ref{}. 

%models that perform NER through token classification.

%We explore 12 different formats that are categorized into the table \ref{tab:formats}. Formats are categorized according to the \emph{Entity Representation} that should be extracted and the \emph{Modality} . 

% distinct formats listed in Table \ref{tab:formats}.


% \ac{your table appears very low (2 pages late) and is very not self explaining}
% Those are categorized based on the type of entity representation to be extracted and the corresponding modality. \ac{unclear: c'est quoi modality ? En plus ici tu parles du "type of entity" mais je crois que ce n'est pas le type au sens NER, si ?}

%that we decided to avoid due to the poor performance of these formats in the initi al results.


% \pe{Should we speak about data leakage?}\ma{yes in the limitation}

% \pe{Should we define each format.}\ma{if you have a reference for that refer to it, if not define :) or if we can simply explain each of them while motivating them in a few words?}

% \begin{table*}[ht]
% \begin{center}
% \begin{tabular}{llll|lll}
% \toprule
%   &  \multicolumn{3}{c|}{\textbf{Entity Representation}}& \multicolumn{3}{c}{\textbf{Modality}} \\  \midrule
%  \textbf{Formats} &  \parbox{2.25cm}{Text \\ Reconstruction}  & \parbox{1.7cm}{String \\ Extraction} & \parbox{1.7cm}{Span \\ Extraction}& Multi &  Single & Conversational  \\ %& Parsing
%  \midrule
% \textbf{multi\_bio}    & \checkmark &  &  & \checkmark &  &   \\ \hline %& mid
% \textbf{multi\_brat}   &            &  \checkmark  &  \checkmark  &  \checkmark  &  &   \\ %& easy
% \textbf{multi\_code}   &            &  \checkmark  &  &  \checkmark  &  &    \\  %& easy
% \textbf{multi\_span}   &            &  &  \checkmark  &  \checkmark  &  &   \\ %&  easy
% \textbf{multi\_tag}    & \checkmark &  &  &  \checkmark  &  &    \\  %& hard
% \textbf{multi\_term}   &            &  \checkmark  &  &  \checkmark  &  &    \\  %& easy
% \textbf{multi\_triple} &            &  \checkmark  &  &  \checkmark  &  &     \\  %&  easy
% \textbf{single\_code}  &            &  \checkmark  &  &  &  \checkmark  &    \\  %&  easy
% \textbf{single\_span}  &            &  &  \checkmark  &  &  \checkmark  &     \\  %& easy
% \textbf{single\_tag}   & \checkmark &  &  &  &  \checkmark  &   \\  %& hard
% \textbf{single\_term}  &            &  \checkmark  &  &  &  \checkmark  &     \\  %& easy
% \textbf{conv\_term}    &            &  \checkmark  &  &  &  &  \checkmark     \\  %& easy
% \bottomrule
% \end{tabular}
% \caption{Summary of the categorization of the different formats used.}
% \label{tab:formats}
% \end{center}
% \end{table*}

% \ma{do we need the following paragraph}
% We applied minimal preprocessing to each dataset. When necessary, we realigned the annotation spans. For the PGx and CADEC datasets, we split each example into individual lines, treating each line as a separate example. Additionally, for CADEC, we pre-tokenized the text to ensure consistency with the other datasets. This was done using a simplified custom version of the TreebankWordTokenizer \cite{bird2006nltk}. We verified that the pre-tokenization process did not alter any entity boundaries. An example of the pre-tokenization is shown below:

% \begin{itemize}
%     \item Before: "Some stomach irritation, feels a bit like my pressure is up (in my head mostly)."
%     \item After: "Some stomach irritation , feels a bit like my pressure is up ( in my head mostly ) ."
% \end{itemize}

% To verify data integrity, we assessed all format conversions across datasets, confirming that no changes occurred during conversion or subsequent reversion. We end up with 6 inconsistency. 
%  % \ma{this part can go if more space is needed since it is very basic}
